Non-linear dependence and Granger causality: A vine copula approach

Inspired by Jang et al. (2022), we propose a Granger causality-in-the-mean test for bivariate $k-$Markov stationary processes based on a recently introduced class of non-linear models, i.e., vine copula models. By means of a simulation study, we show that the proposed test improves on the statistical properties of the original test in Jang et al. (2022), and also of other previous methods, constituting an excellent tool for testing Granger causality in the presence of non-linear dependence structures. Finally, we apply our test to study the pairwise relationships between energy consumption, GDP and investment in the U.S. and, notably, we find that Granger-causality runs two ways between GDP and energy consumption.

==> tables.tex <==
\begin{tblr}{
  row{1} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=3}{},
  cell{1}{5} = {c=3}{},
  cell{1}{8} = {c=3}{},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{3}{10} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{4}{7} = {c},
  cell{4}{8} = {c},
  cell{4}{9} = {c},
  cell{4}{10} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{5}{7} = {c},
  cell{5}{8} = {c},
  cell{5}{9} = {c},
  cell{5}{10} = {c},
  vline{5,8} = {2-5}{},
  hline{1,3,6} = {-}{},
  hline{2} = {2-10}{},
}
Model & T=50   &                                  &        & T=100  &                                  &        & T=200  &                                  &        \\
      & M-vine & Jang et al. & Linear & M-vine & Jang et al. & Linear & M-vine & Jang et al. & Linear \\
S1    & 0.046  & 0.066                            & 0.058  & 0.050  & 0.070                            & 0.048  & 0.056  & 0.050                            & 0.058  \\
S2    & 0.044  & 0.052                            & 0.058  & 0.052  & 0.080                            & 0.054  & 0.062  & 0.066                            & 0.056  \\
S3    & 0.058  & 0.070                            & 0.060  & 0.054  & 0.054                            & 0.052  &    0.050    &                     0.070             &    0.046    
\end{tblr}


\begin{tblr}{
  row{1} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=3}{},
  cell{1}{5} = {c=3}{},
  cell{1}{8} = {c=3}{},
  cell{3}{2} = {c},
  cell{3}{3} = {c},
  cell{3}{4} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{3}{7} = {c},
  cell{3}{8} = {c},
  cell{3}{9} = {c},
  cell{3}{10} = {c},
  cell{4}{2} = {c},
  cell{4}{3} = {c},
  cell{4}{4} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{4}{7} = {c},
  cell{4}{8} = {c},
  cell{4}{9} = {c},
  cell{4}{10} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{4} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{5}{7} = {c},
  cell{5}{8} = {c},
  cell{5}{9} = {c},
  cell{5}{10} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{4} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{6}{7} = {c},
  cell{6}{8} = {c},
  cell{6}{9} = {c},
  cell{6}{10} = {c},
  vline{3,6,9} = {1}{},
  vline{5,8} = {2-6}{},
  hline{1,3,7} = {-}{},
  hline{2} = {2-10}{},
}
Model & T=50   &       &        & T=100  &       &        & T=200  &       &        \\
      & M-vine & Jang et al.  & Linear & M-vine & Jang et al.      & Linear & M-vine & Jang et al.      & Linear \\
P1    & 0.706  & 0.630 & 0.958  & 0.916  & 0.856 & 1.000  & 0.996  & 0.978 & 1.000  \\
P2    & 0.544  & 0.442 & 0.802  & 0.720  & 0.676 & 0.982  & 0.942 &  0.886 & 1.000  \\
P3    & 0.430  & 0.238 & 0.348  & 0.716  & 0.384 & 0.388  & 0.986  & 0.644 & 0.392  \\
P4    & 0.684  & 0.426 & 0.530  & 0.972  & 0.628 & 0.518  & 1.000  & 0.950 & 0.508  
\end{tblr}
